ToKen: Task Decomposition and Knowledge Infusion for Few-Shot Hate Speech Detection

Hate speech detection is complex; it relies on commonsense reasoning, knowledge of stereotypes, and an understanding of social nuance that differs from one culture to the next. It is also difficult to collect a large-scale hate speech annotated dataset. In this work, we frame this problem as a few-shot learning task, and show significant gains with decomposing the task into its "constituent" parts. In addition, we see that infusing knowledge from reasoning datasets (e.g. Atomic2020) improves the performance even further. Moreover, we observe that the trained models generalize to out-of-distribution datasets, showing the superiority of task decomposition and knowledge infusion compared to previously used methods. Concretely, our method outperforms the baseline by 17.83% absolute gain in the 16-shot case.

==> ToKen LaTeX/tables/atomic_templates.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}
\begin{tabular}{@{}p{0.28\linewidth}p{0.65\linewidth}@{}}
\toprule
\textbf{Relation} & \textbf{Human Readable Template}                  \\ \midrule
ObjectUse          & \{0\} is used for \{1\}                           \\
AtLocation         & You are likely to find \{0\} in \{1\}             \\
MadeUpOf           & \{0\} is made up of \{1\}                         \\
HasProperty        & \{0\} is \{1\}                                    \\
CapableOf          & \{0\} can \{1\}                                   \\
Desires            & \{0\} wants \{1\}                                 \\
NotDesires         & \{0\} does not want \{1\}                         \\
isAfter            & Something that happens after \{0\} is \{1\}       \\
HasSubEvent        & Something you might do while \{0\} is \{1\}       \\
isBefore           & Something that happens before \{0\} is \{1\}      \\
HinderedBy         & \{0\} is hindered by \{1\}                        \\
Causes             & Sometimes \{0\} causes \{1\}                      \\
xReason            & \{0\}. The reason for PersonX doing this is \{1\} \\
isFilledBy         & \{0\} can be filled by \{1\}                      \\
xNeed              & But before \{0\}, PersonX needed \{1\}            \\
xAttr              & \{0\} is seen as \{1\}                            \\
xEffect            & As a result of \{0\}, PersonX will \{1\}          \\
xReact             & As a result of \{0\}, PersonX feels \{1\}         \\
xWant              & After \{0\}, PersonX would want \{1\}             \\
xIntent            & Because of \{0\}, PersonX wanted \{1\}            \\
oEffect            & as a result of \{0\}, others will \{1\}           \\
oReact             & as a result of \{0\}, others would feel \{1\}     \\
oWant              & as a result of \{0\}, others would want \{1\}     \\ \bottomrule
\end{tabular}
\caption{Human readable templates for each relation used to train the BART model. The \texttt{Head} is injected in place of \{0\} and is tasked with predicting the \texttt{Tail} \{1\} in a conditional generation framework.}
\label{tab:atomic_templates}
\end{table}

==> ToKen LaTeX/tables/hate_speech_position.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Order}               & \textbf{16}      & \textbf{32}      & \textbf{64}      & \textbf{128}     & \textbf{256}     & \textbf{512}     & \textbf{1024}    \\ \midrule
OFF GD GI \textbf{HS}           & \textbf{55.60}         & \textbf{62.31}          & \textbf{68.47}          & 69.22          & 69.64          & 70.49          & 71.69 \\
OFF GD \textbf{HS} GI  & 54.67          & 60.36          & 68.02          & 67.65          & 68.66          & 70.13          & 70.92          \\
OFF \textbf{HS} GD GI & 54.53         & 56.14            & 67.02          & 68.59           & \textbf{71.37}               & \textbf{72.47} & \textbf{72.39}          \\ 
\textbf{HS} OFF GD GI & 51.64         & 62.04           & 64.48           & \textbf{69.45}           & 70.33            & 71.33   & 72.20          \\ \midrule

GD GI \textbf{OFF} HS & 38.28          & 27.11          & 31.32          & 53.98          & 52.12          & 60.69          & 67.20   \\ \bottomrule
\end{tabular}
\caption{The validation performance of the best model on the HS detection task as a function of the position of the HS label in the sequence of subtasks across different number of training samples.}
\label{tab:hs_pos_results}
\end{table*}

==> ToKen LaTeX/tables/implications.tex <==
\begin{table}
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{\# of Samples} & \textbf{Baseline} & \textbf{\token} & \textbf{+Impl} \\ \midrule
\textbf{16}            & 52.67           & 58.21           & 57.02                \\
\textbf{32}            & 52.71           & 64.47           & 59.98                \\
\textbf{64}            & 57.60           & 70.93           & 65.50                \\
\textbf{128}           & 60.01           & 71.25           & 67.89                \\
\textbf{256}           & 66.81           & 71.62           & 69.22                \\
\textbf{512}           & 69.41           & 72.59           & 70.12                \\
\textbf{1024}          & 74.72           & 74.09           & 71.45                \\ \bottomrule
\end{tabular}
\caption{\textbf{Implications Results} The HS detection performance of the \textbf{Baseline} in comparison with the \textbf{Subtasks} models before and after adding the implication to the subtasks across 5 runs for a given training set size.}
\label{tab:implications}
\end{table}

==> ToKen LaTeX/tables/knowledge_infusion.tex <==
\begin{table*}
\centering
\begin{tabular}{@{}llccccccc@{}}
\toprule
\multicolumn{2}{c}{\textbf{Model}}                        & \textbf{16}                 & \textbf{32}                 & \textbf{64}                          & \textbf{128}                         & \textbf{256}                         & \textbf{512}                & \textbf{1024}               \\ \midrule
\multirow{2}{*}{\textbf{BART}}        & \textbf{Baseline} & 45.31                      & 53.23                     & 56.41                             & 60.12                                & 64.37                            & 70.29                    & 73.95           \\
                                      & \textbf{Subtasks} & 58.89                      & 61.77                     & 68.03                            &  70.25                                & 70.28                            & 70.65          & 72.76                      \\ \midrule \midrule
\multirow{2}{*}{\textbf{+ StereoSet}} & \textbf{Baseline} & 53.30                      & 54.68                     & 54.17                              & 61.41                              & 67.69                              & 71.25            & 73.68                     \\
                                      & \textbf{Subtasks} & 42.86                      & \textbf{66.17}            & 69.01                              & 70.06                              & 70.14                              & 72.14                     & 72.64                     \\ \midrule \midrule
\multirow{2}{*}{\textbf{+ \atomic}}     & \textbf{Baseline} & 44.76                      & 49.60                      & 64.89                              & 69.38                              & 70.09                              & 72.32            & \textbf{73.97}                     \\
                                      & \textbf{Subtasks} & \textbf{63.14}             & 62.01                    & 67.96                              & 70.94                              & 70.16                              & 72.29                     & 72.96                     \\ 
\multirow{2}{*}{\textbf{+ StereoSet}} & \textbf{Baseline} & 44.75 & 47.47 & 56.18          & 62.88          & 66.38          & 69.77 & 71.50 \\
                                      & \textbf{Subtasks} & 59.74 & 63.28 & \textbf{70.08} & \textbf{70.99} & \textbf{70.57} & \textbf{72.36} & 73.80 \\ \bottomrule
\end{tabular}
\caption{\textbf{Knowledge Infusion Results} Here we report binary F1-score on the SBIC testing set for the HS detection task using models with different degrees of knowledge infusion. In each row we compare the corresponding baseline and subtasks models. Results in \textbf{bold} show the best overall model in each few-shot setting. See Section \ref{sec:knowledge_infusion} for more details.}
\label{tab:knowledge_infusion_results}
\end{table*}

==> ToKen LaTeX/tables/scale_table.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Model}               & \textbf{16}      & \textbf{32}      & \textbf{64}      & \textbf{128}     & \textbf{256}     & \textbf{512}     & \textbf{1024}    \\ \midrule
\textbf{Baseline}           & 53.49          & 51.47          & 58.28          & \textbf{66.70}         & \textbf{68.24}          & \textbf{70.09}          & \textbf{71.30} \\
\textbf{\token}           & \textbf{55.23}       & \textbf{60.29}         & \textbf{63.68}         & 65.10          & 67.52          & 68.67          & 69.66          \\
\end{tabular}
\caption{Results using BART\textsubscript{BASE} as the core model. Similar to the previous experiments the baseline model predicts the HS label directly, while the \token model employs task decomposition and knowledge infusion using the \atomic and StereoSet datasets. (see $\S$\ref{sec:scale_matter} for more details)}
\label{tab:scale_results}
\end{table*}

==> ToKen LaTeX/tables/task_decomposition.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Model}               & \textbf{16}      & \textbf{32}      & \textbf{64}      & \textbf{128}     & \textbf{256}     & \textbf{512}     & \textbf{1024}    \\ \midrule
\textbf{Baseline}           & 45.31          & 53.23          & 56.41          & 60.12          & 64.37          & 70.29          & \textbf{73.95} \\
% \textbf{+ Offensiveness}     & 46.69          & 56.41          & 57.01          & 59.28          & 61.89          & 71.46          & 72.63          \\
\textbf{Minimal Decomposition}  & 50.79          & 56.12          & 56.46          & 59.78          & 64.94          & 67.83          & 69.95          \\
\textbf{+ Group Identification} & \textbf{58.89} & \textbf{61.77} & \textbf{68.03} & \textbf{70.25} & \textbf{70.28} & \textbf{70.65} & 72.76          \\ \bottomrule
\end{tabular}
\caption{Results of the Task Decomposed Model on the \textit{Hate Speech} detection task (Binary F1-score). \textbf{Baseline} predicts only whether the input post is HS or not. \textbf{Minimal Decomposition} additionally predicts whether the post is offensive or not and the group detection. \textbf{+ Group Identification} additionally predicts the minority groups the post is targeting if any. }
\label{tab:task_decomposed_results}
\end{table*}
